The Curse of Passive Data Collection in Batch Reinforcement Learning

In high stake applications, active experimentation may be considered too risky and thus data are often collected passively. While in simple cases, such as in bandits, passive and active data collection are similarly effective, the price of passive sampling can be much higher when collecting data from a system with controlled states. The main focus of the current paper is the characterization of this price. For example, when learning in episodic finite state-action Markov decision processes (MDPs) with $\mathrm{S}$ states and $\mathrm{A}$ actions, we show that even with the best (but passively chosen) logging policy, $\Omega(\mathrm{A}^{\min(\mathrm{S}-1, H)}/\varepsilon^2)$ episodes are necessary (and sufficient) to obtain an $\epsilon$-optimal policy, where $H$ is the length of episodes. Note that this shows that the sample complexity blows up exponentially compared to the case of active data collection, a result which is not unexpected, but, as far as we know, have not been published beforehand and perhaps the form of the exact expression is a little surprising. We also extend these results in various directions, such as other criteria or learning in the presence of function approximation, with similar conclusions. A remarkable feature of our result is the sharp characterization of the exponent that appears, which is critical for understanding what makes passive learning hard.

==> checklist.tex <==
%!TEX root =  main.tex

\section*{Checklist}

\if0
%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%
\fi

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See \cref{sec:lb} and \cref{sec:ub}}
  \item Did you describe the limitations of your work?
    \answerYes{See \cref{sec:related}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See the problem set up \cref{sec:BPO} and the statement of the results}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{See the supplementary material}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNA{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> intro_old.tex <==
%!TEX root =  main.tex
\section{Introduction}

Batch reinforcement learning (RL) broadly refers to
the problem of finding a policy with high expected return in a stochastic control problem
when only a batch of data collected from the controlled system is available.
Here, we consider this problem for finite state-action (``tabular'') Markov decision processes (MDPs)
when the data takes the form of trajectories obtained by following some logging policy.
In more details, the trajectories are composed of sequences of states, actions, and rewards, where the action is chosen by the logging policy and the next state and rewards follow the distributions specified by the MDP's transition parameters.
Arguably, this is the most natural problem setting to consider in batch learning.
The basic questions are {\em (a)} what logging policy should one choose to generate the data so as to maximize the chance of obtaining a good policy with as little data as possible; and {\em (b)} how many transitions are sufficient and necessary to obtain a good policy and which algorithm to use to obtain such a policy? Note that here the logging policy needs to be chosen \emph{a priori}, that is, before the data collection process begins. An alternative way of saying this is that the data collection is done in a passive way.

Our main results are as follows:
First, we show that (perhaps unsurprisingly), in the lack of extra information about the nature of the MDP, the best logging policy should choose actions \emph{uniformly at random}. 
Next, we show that the number of transitions necessary and sufficient to obtain a good policy, \emph{the sample complexity of learning}, is an exponential function of the minimum of the number of states and the planning horizon. 
In particular, we prove that the sample complexity of obtaining $\epsilon$-optimal policies is at least $\Omega(\rA^{\min(\rS-1, H+1)})$ for $\gamma$-discounted problems, where $\rS$ is the number of states, $\rA$ is the number of actions, and $H$ is the effective horizon defined as 
$H=\lfloor \tfrac{\ln(\sfrac{1}{\epsilon})}{\ln(\sfrac1\gamma)} \rfloor$;
and it is at least $\Omega(\rA^{\min(\rS-1, H)}/\varepsilon^2)$ for finite horizon problems, where $H$ is the planning horizon of the problem.  
% In particular, our lower bound shows that the sample complexity for obtaining $\epsilon$-optimal policies is at least $\Omega( \rA^{\min(\rS-1, H+1)}/f(\epsilon))$ 
% where $\rS$ is the number of states, $\rA$ is the number of actions and $H$ is the planning horizon, 
% which matches the horizon in fixed horizon problems, and is defined as
% $H=\lfloor \tfrac{\ln(\sfrac{1}{\epsilon})}{\ln(\sfrac1\gamma)} \rfloor$ 
% for discounted problems with discount factor $\gamma$ in which case $f(\varepsilon)=1$, while in finite horizon problems $f(\varepsilon)=\varepsilon^2$. 
We also prove an upper bound for the plug-in algorithm that essentially matches our lower bound.
These results are complemented with a lower bound that shows that in the average reward case the sample complexity is infinite.
%  (for details of our results, see \cref{sec:results}).

The main advances that our work represents over prior works are as follows:
First, our results show that 
for finite (effective) horizons,
the \emph{sample complexity is finite}.
In contrast, existing results available for the closely related setting of batch (or off-policy) policy evaluation (e.g., \citet{uehara2021finite, ren2021nearly} and references therein)
depend on visitation probability ratios computed for the target and the logging policies, which leave open the possibility of infinite sample complexity even for policy evaluation.
The infinite sample complexity is in fact unavoidable when the logging policy is poorly chosen, i.e., when it does not even sample some actions in some states.
As expected, the best control in the uninformed case is achieved by the uniform policy, for which the said ratio of state-action marginals after $t$ steps can be shown to be at most $\rA^{t+1}$
%$(SA)^t$ 
%(cf. \cref{sec:absratiobound} for the brief argument that shows this).
(cf. Appendix A for the brief argument that shows this).
Based on this, we expect a sample complexity that scales with $\rA^{H+1}$ where $H$ is the (effective) horizon, and indeed this is what our result shows when the number of states $\rS$ is large.
%While this crude bound predicts an unbounded sample complexity for infinite horizon problems, 
%While this crude bound predicts that the base of the exponential dependence includes the number of states, 
%our direct analysis shows that this dependence can be avoided even though policy optimization is expected to be a harder problem than policy evaluation. 
Our sample complexity upper bound is shown for any ``plug-in method'' and the analysis is inspired by \citet{agarwal2020model}, although with some essential differences, stemming from the different setting.
Our lower bound that shows that the sample complexity for average reward problems is infinite highlights that an (effective) finite planning horizon is key for bounded sample complexity.

A second highlight of our result is that it implies an exponential gap between the sample complexity of learning from policy-induced data and other forms of learning. 
A similar conclusion is drawn in the recent paper of \citet{zanette2020exponential}, which served as the main motivation for our work. 
\citeauthor{zanette2020exponential} demonstrated an exponential separation for the case when batch learning is used in the presence of linear function approximation. A careful reading of their paper shows that the lower bound shown there does not apply to the tabular setting that we consider in the present work. Hence, our work can be seen as a strengthening of the exponential separation result of 
\citeauthor{zanette2020exponential}, as the tabular case is arguably more fundamental 
than the case when a function approximator is involved. In effect, our results show that the exponential separation is not connected to whether a function approximation needs to be used, but appears as soon as the learner is restricted to use data that comes in the form of trajectories obtained by following a policy.
%While the question studied in this paper is fundamental
For further details on the relationship of our work to previous work, see \cref{sec:related}.

Our result can be seen as contributing an argument for that when the goal is to learn a controller in a feedback situation, learning from passively logged data has some distinct disadvantage over learning in a closed loop, interactive fashion. As specific examples, one can ask how critical it is to let a conversational dialogue system interact with humans while being trained, or can good conversational assistants be built by  training them on text available on the web? Similarly, one can ask the same question in the context of training controllers to build self-driving cars? The exponential separation shown for the very simple setting of finite Markov decision processes shows that it may be overly optimistic to believe that good policies can be acquired by patching together fragments of logged trajectories. 
Here, it is also important to remember that the exponential separation only happens as the planning horizon grows, showing that learning a good policy which implies a distribution shift can be significantly more challenging than just to learning to predict well with no distribution shift. Thus, in settings where the planning horizon is large, the role of learning interactively should not be underestimated.


